"A Party That Never Stops": Designing Digital Third Places for Young People's Friendships on Discord

Third places---informal settings where relationships grow through repeated casual contact---are increasingly inaccessible to young people. Prior work shows that virtual third places exist, but little is known about how persistent settings and control over participation work together as relationships form. We interviewed 25 active Discord users ages 15--24 who had reported forming at least one friendship on the platform. Their accounts highlighted two conditions that worked together. Persistent, socially legible servers let them return to the same community, recognize others, and build shared histories and norms. Controllable presence let them observe, participate, deepen a relationship, or withdraw while managing visibility, identity, and commitment. Graduated visibility was especially important for cautious entry and identity exploration. We translate these findings into design principles, showing how each can support some of Oldenburg's third-place functions while creating tensions with others. These findings suggest that persistent digital communities can complement increasingly scarce physical third places by giving young people recurring, low-pressure opportunities for social connection.

==> formatting/dev-commands.tex <==
%!TEX root = main.tex

%%
%% Note: This file includes all new commands that are needed for the preliminary 
%% paper-writing (draft / review) stage of the paper. These commands should NOT
%% be included in the camera-ready version of the paper.
%%
%% All content in this file should take at least one argument. Custom commands 
%% for simple aliases should be provided in "dev-aliases.tex".
%%

%% Note: Custom colors for in-paper comments
\definecolor{LIGHTPINK}{RGB}{237,157,202}
\definecolor{LIGHTRED}{RGB}{210,121,121}
\definecolor{LIGHTORANGE}{RGB}{230,170,50}
\definecolor{LIGHTGOLD}{RGB}{210,194,121}
\definecolor{LIGHTGREEN}{RGB}{121,210,121}
\definecolor{LIGHTAQUA}{RGB}{121,206,210}
\definecolor{LIGHTBLUE}{RGB}{121,124,210}
\definecolor{LIGHTPURPLE}{RGB}{153,102,255}
\definecolor{RED}{RGB}{178,34,34}
\definecolor{GRAY}{RGB}{166,166,166}
\definecolor{WHITE}{RGB}{255,255,255}

%% Note: General TODO and cut commands
\newcommand{\todo}[1]{
    \addcontentsline{toc}{subsection}{  %
        \protect\numberline{}           % Align text appropriately
        \textcolor{RED}{[TODO] #1}}     % Add todo to the table of contents
    \textcolor{RED}{[TODO] \emph{#1}}}  % Typeset the todo note in the text
\newcommand{\cut}[1]{\textcolor{RED}{\st{#1}}}

\renewcommand{\cut}[1]{\textcolor{RED}{\st{#1}}}

%%
%% Note: Labeled in-paper comments for collaborators (with and without underlined
%% text). Each author should specify a new command for their name with a
%% different comment color, using the example new command for \jane below. 
%% Alternatively, authors can use the more complicated \guest command, but must
%% provide their name each time they leave a comment.
%%

%% Usage: \jane[(OPTIONAL) Text to underline in square brackets]{Comment.}
\newcommandx{\jane}[2][1=] 
    {\setulcolor{LIGHTGREEN}{\ul{#1}} \textcolor{LIGHTGREEN}
    {[\textbf{Jane:} #2]}}
%% Usage: \guest[(OPTIONAL) Text to underline]{Name}{Comment text}
\newcommandx{\guest}[3][1=]
    {\setulcolor{LIGHTORANGE}{\ul{#1}} \textcolor{LIGHTORANGE} 
    {[\textbf{#2:} #3]}}

%%
%% Note: Custom status badges can be added to sections and subsections to label 
%% which ones are ready (or not) for feedback to facilitate collaboration amongst
%% authors. Badges should be added directly to the section heading.
%%
\newcommand{\badge}[2]{\colorbox{#1}{\small\textcolor{WHITE}{\texttt{#2}}}}
\newcommand{\headerBadge}[2]{\hspace*{\fill}\badge{#1}{#2}}

\newcommand{\locked}{\headerBadge{LIGHTPURPLE}{locked}}
\newcommand{\complete}{\headerBadge{LIGHTBLUE}{complete}}
\newcommand{\feedbackProvided}{\headerBadge{LIGHTGREEN}{feedback provided}}
\newcommand{\readyForFeedback}{\headerBadge{LIGHTORANGE}{feedback requested}}
\newcommand{\underRevision}{\headerBadge{LIGHTRED}{under revision}}
\newcommand{\incomplete}{\headerBadge{RED}{incomplete}}


